Continual Learning with Weight Interpolation

Continual learning poses a fundamental challenge for modern machine learning systems, requiring models to adapt to new tasks while retaining knowledge from previous ones. Addressing this challenge necessitates the development of efficient algorithms capable of learning from data streams and accumulating knowledge over time. This paper proposes a novel approach to continual learning utilizing the weight consolidation method. Our method, a simple yet powerful technique, enhances robustness against catastrophic forgetting by interpolating between old and new model weights after each novel task, effectively merging two models to facilitate exploration of local minima emerging after arrival of new concepts. Moreover, we demonstrate that our approach can complement existing rehearsal-based replay approaches, improving their accuracy and further mitigating the forgetting phenomenon. Additionally, our method provides an intuitive mechanism for controlling the stability-plasticity trade-off. Experimental results showcase the significant performance enhancement to state-of-the-art experience replay algorithms the proposed weight consolidation approach offers. Our algorithm can be downloaded from https://github.com/jedrzejkozal/weight-interpolation-cl.

==> images/schema.tex <==
\begin{tikzpicture}[node distance=0.6cm, auto,
trapezenode/.style={trapezium, trapezium angle=75, very thick, minimum width=15mm, rotate=-90},
% imagenode/.style={trapezium, trapezium left angle=60, trapezium right angle=-60, minimum width=1.6cm, minimum height=0.5cm, ultra thin, fill=white!5, draw}
imagenode/.style={rectangle, minimum width=1.0cm, minimum height=1.0cm, ultra thin, fill=white!5, draw}
]

% anchors
\node[] (anchor_old_network) {};
\node[] (anchor_training) [right=2.0cm of anchor_old_network] {};
\node[] (anchor_model_trained) [right=3cm of anchor_training] {};
\node[] (anchor_interpolation) [right=2cm of anchor_model_trained] {};
\node[] (anchor_trained_model) [right=3cm of anchor_interpolation] {};

% told_network.soutask border anchors
\node[] (anchor_task_left_upper) [left=1.5cm of anchor_old_network] {};
\node[] (anchor_task_left_lower) [below=6cm of anchor_task_left_upper] {};
\node[] (anchor_task_right_upper) [right=13cm of anchor_task_left_upper] {};
\node[] (anchor_task_right_lower) [below=6cm of anchor_task_right_upper] {};

% nodes
\node[trapezenode, draw] (old_network) [below=1cm of anchor_old_network] {$\theta_P$};
\node[rectangle, draw, very thick, minimum width=2.0cm] [below=0.7cm of anchor_training] (training) {training};
\node[trapezenode, draw] [below=1cm of anchor_model_trained] (trained_network) {$\theta$};
\node[rectangle, draw, very thick] [below=0.7cm of anchor_interpolation] (interpolation) {interpolation};
\node[trapezenode, draw] [below=1cm of anchor_trained_model] (trained_model) {$\theta_t$};

% image batch old rehearsal
\node (anchor_img1) [left=0.5cm of anchor_old_network] {};
\node (anchor_img2) [right=0.05cm of anchor_img1] {};
\node (anchor_img3) [right=0.05cm of anchor_img2] {};
\node[imagenode] [below=3.8cm of anchor_img3] (image_A_3) {};
\node[imagenode] [below=3.9cm of anchor_img2] (image_A_2) {};
\node[imagenode] [below=4.0cm of anchor_img1] (image_A_1) {};
\node [below=0.1cm of image_A_1] (memory_buffer) {memory buffer $\mathcal{M}$};

% image batch new data
\node (anchor_img1_new) [right=1.8cm of anchor_old_network] {};
\node (anchor_img2_new) [right=0.05cm of anchor_img1_new] {};
\node (anchor_img3_new) [right=0.05cm of anchor_img2_new] {};
\node[imagenode] [below=2.3cm of anchor_img3_new] (image_A_3_new) {};
\node[imagenode] [below=2.4cm of anchor_img2_new] (image_A_2_new) {};
\node[imagenode] [below=2.5cm of anchor_img1_new] (image_A_1_new) {};
\node [below=0.1cm of image_A_1_new] (new_data) {new data};

% image batch update buffer
\node (anchor_img1_new_buffer) [right=3.8cm of anchor_old_network] {};
\node (anchor_img2_new_buffer) [right=0.05cm of anchor_img1_new_buffer] {};
\node (anchor_img3_new_buffer) [right=0.05cm of anchor_img2_new_buffer] {};
\node[imagenode] [below=3.8cm of anchor_img3_new_buffer] (image_A_3_new_buffer) {};
\node[imagenode] [below=3.9cm of anchor_img2_new_buffer] (image_A_2_new_buffer) {};
\node[imagenode] [below=4.0cm of anchor_img1_new_buffer] (image_A_1_new_buffer) {};
\node [below=0.1cm of image_A_1_new_buffer] (memory_buffer_new) {updated buffer $\mathcal{M}$};


% task borders
\draw[dotted] (anchor_task_left_upper) -- (anchor_task_left_lower);
\draw[dotted] (anchor_task_right_upper) -- (anchor_task_right_lower);

% node connections
\node[] (anchor_left) [left=2cm of anchor_old_network] {};
\node[] (anchor_left_lower) [below=0.9cm of anchor_left] {};
\draw[->] (anchor_left_lower) -- (old_network.south);

\node[] (anchor_left_llower) [below=3.1cm of anchor_left_lower] {};
\draw[->] (anchor_left_llower) -- (image_A_2);

\node[] (anchor_right) [right=12cm of anchor_old_network] {};
\node[] (anchor_right_lower) [below=0.9cm of anchor_right] {};
\draw[->] (trained_model) -- (anchor_right_lower) {};

\node[] (anchor_left_rright) [below=3.1cm of anchor_right_lower] {};
\draw[->] (image_A_2_new_buffer) -- (anchor_left_rright);

\draw[->] (old_network.north) -- (training.west);
\draw[->] (training.east) -- (trained_network.south);
\draw[->] (trained_network.north) -- (interpolation.west);
\draw[->] (interpolation.east) -- (trained_model.south);
% \draw[->] (trained_model.south) -- (

\draw[->] (image_A_2) -- (image_A_2_new_buffer);

% task annotations
\node (anchor_current_task) [right=5.0cm of anchor_old_network] {};
\node (current_task) [below=6.0cm of anchor_current_task] {task $t$};
\node (anchor_prev_task) [left=3.0cm of anchor_old_network] {};
\node (prev_task) [below=6.0cm of anchor_prev_task] {task $t-1$};
\node (anchor_next_task) [right=12.5cm of anchor_old_network] {};
\node (next_task) [below=6.0cm of anchor_next_task] {task $t+1$};

\draw[->] (image_A_2) -- (training);
\draw[->] (image_A_2_new) -- (training);
\draw[->] (image_A_2_new.east) -- (image_A_2_new_buffer.north);
\draw[->] (image_A_2_new_buffer.east) -- (interpolation.south);

\end{tikzpicture}

==> tables/eval_n_tasks.tex <==
\begin{tabular}{c|c|c|c}
    \hline
    method & 5 tasks & 10 tasks & 20 tasks \\
    \hline
     Joint      & 70.75±0.4098  & 70.536±0.7548 & 70.362±0.6467 \\
     Finetuning & 17.054±0.3718 & 9.068±0.1015  & 4.684±0.1157  \\
     oEWC        & -             & 8.864±0.512  & 4.588±0.2373  \\
     SI         & -             & -             & -             \\
     iCARL      & 54.994±0.1608 & 46.914±0.6579 & 32.792±1.3162 \\
     ER         & 29.036±0.9771 & 22.452±1.2624 & 16.81±1.272   \\
     aGEM       & -             & 9.172±0.176   & 4.706±0.1038  \\
     BIC        & 53.924±1.0652 & 37.554±1.6439 & 23.846±2.0151 \\
     ER-ACE     & 44.882±0.5717 & 37.754±1.2281 & 31.302±0.8632 \\
     GDumb      & 9.568±0.5151  & 9.986±0.6782  & 10.25±0.6153  \\
     MIR        & 29.146±0.7147 & 21.958±1.1339 & 16.548±1.5982 \\
     % LUCIR      &  &  &  \\
     DER        & 42.872±1.2522 & 36.64±1.5853  & 28.412±1.7216 \\
     xDER       & 54.88±0.3746  & 47.784±0.2916 & 40.724±0.3933 \\
     \hline
     ER + CLeWI      & 43.384±0.7125 & 40.31±1.0762  & 33.58±0.4273  \\
     aGEM + CLeWI & -             & 22.754±1.4103 & -             \\
     BIC + CLeWI &  &  &  \\
     ER-ACE + CLeWI & - & 36.968±0.5544 & - \\ % 10 tasks hyperparameters initial value : 38.53
     GDumb + CLeWI &  &  &  \\
     MIR + CLeWI & -             & 40.058±0.8381 & -             \\
     % LUCIR + CLeWI &  &  &  \\
     DER++ + CLeWI & -             & 38.16±1.8646  & -             \\
    \hline
\end{tabular}
